Enhancing Out-of-Distribution Detection in Natural Language Understanding via Implicit Layer Ensemble

Out-of-distribution (OOD) detection aims to discern outliers from the intended data distribution, which is crucial to maintaining high reliability and a good user experience. Most recent studies in OOD detection utilize the information from a single representation that resides in the penultimate layer to determine whether the input is anomalous or not. Although such a method is straightforward, the potential of diverse information in the intermediate layers is overlooked. In this paper, we propose a novel framework based on contrastive learning that encourages intermediate features to learn layer-specialized representations and assembles them implicitly into a single representation to absorb rich information in the pre-trained language model. Extensive experiments in various intent classification and OOD datasets demonstrate that our approach is significantly more effective than other works.

==> assets/tab/selective_ensemble.tex <==
\begingroup
\setlength{\tabcolsep}{11pt} % Default value: 6pt
\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{l|c|c|c}
        \toprule
        \multicolumn{1}{c|}{\multirow{2}{*}{Models}} &\multicolumn{1}{c|}{\multirow{2}{*}{Acc}}& \multicolumn{2}{c}{Cosine} \\ \cline{3-4}
         &  &\multicolumn{1}{l|}{AUROC} & \multicolumn{1}{l}{FPR@95} \\
         \midrule
            LaCL (variant 1) & \textbf{95.72} & 92.51 & 37.34\\
            LaCL (variant 2) & 95.52 & 92.55 & 38.71\\
            LaCL (original) & 95.66 & \textbf{92.84} & \textbf{35.13}\\
        \bottomrule
        \end{tabular}
    }
    % \vspace{-0.2cm}
    \caption{\textcolor{red}{caption caption caption}}
    \label{tab:selective-ensemble}
\end{table}
\endgroup
